IVOA: Introspective Vision for Obstacle Avoidance

Vision, as an inexpensive yet information rich sensor, is commonly used for perception on autonomous mobile robots. Unfortunately, accurate vision-based perception requires a number of assumptions about the environment to hold -- some examples of such assumptions, depending on the perception algorithm at hand, include purely lambertian surfaces, texture-rich scenes, absence of aliasing features, and refractive surfaces. In this paper, we present an approach for introspective vision for obstacle avoidance (IVOA) -- by leveraging a supervisory sensor that is occasionally available, we detect failures of stereo vision-based perception from divergence in plans generated by vision and the supervisory sensor. By projecting the 3D coordinates where the plans agree and disagree onto the images used for vision-based perception, IVOA generates a training set of reliable and unreliable image patches for perception. We then use this training dataset to learn a model of which image patches are likely to cause failures of the vision-based perception algorithm. Using this model, IVOA is then able to predict whether the relevant image patches in the observed images are likely to cause failures due to vision (both false positives and false negatives). We empirically demonstrate with extensive real-world data from both indoor and outdoor environments, the ability of IVOA to accurately predict the failures of two distinct vision algorithms.

==> evaluation.tex <==
\section{EVALUATION} \label{evaluation}

\mypara{Dataset}We use the Clearpath Jackal, a mobile robot with a skid-steer drive system, for data collection. The robot is equipped with a stereo pair of Point Grey cameras that record $960 \times 600$ images at a rate of $30Hz$. Obstacle detection ground truth is provided by a Kinect depth sensor that is mounted on the robot and captures depth images at a rate of $30Hz$. The cameras and the Kinect are extrinsically calibrated with respect to each other. The robot is driven using a joystick and the captured RGB and depth images by the stereo cameras and the Kinect are logged at full frame rate. The data is then processed offline: the depth images are converted to pointclouds and synchronized with the stereo camera images. For each set of synchronized images the perception module and the Kinect-based monitoring system are queried to determine whether a set of $(x, y, 0)$ points on a 2D grid in front of the robot and on the ground plane are obstacle free or not within a radius of $10cm$. The corresponding pixel coordinates of the query points on the left camera's image plane along with the obstacle detection results are stored to form the dataset. An indoor dataset including XXX image frames and more than XXX traversed by the robot is collected in different buildings with different types of tiling and carpet. An outdoor dataset is also collected, which includes more than XXX traversed by the robot on different surfaces such as asphalt, concrete, and tile in both dry and wet conditions. 



\mypara{Evaluation Metric} The performance of the introspection model is evaluated based on its ability to predict the behavior of the perception model. For each image the introspection model is queried with the same points on the image, for which we have the  prediction result of the perception system as one of the four classes of FP, FN, TP, and TN. The accuracy of the model in predicting each of these classes is assessed as a measure of its performance. Fig.~\ref{fig:evaluation_metric} denotes an example of comparing the output of the introspection model against the ground truth.



\begin{figure}[t]
  \centering 
  \includegraphics[width=0.8\linewidth,trim=0 0 0 0,clip]{fig/evaluationMetric_00004_0000002066_l.jpg}
  \caption{Comparing the ground truth label of the points on a 2D grid with the predicted labels by the introspection model. For each point on the grid, the inner circle's color represents the prediction of the introspection model about the performance of the perception model and the outer one indicates the ground truth result of the perception system.}
  \label{fig:evaluation_metric}
  \vspace{-3mm}
\end{figure}
